On the Semantic Overlap of Operators in Stream Processing Engines

Stream processing is extensively used in the IoT-to-Cloud spectrum to distill information from continuous streams of data. Streaming applications usually run in dedicated Stream Processing Engines (SPEs) that adopt the DataFlow model, which defines such applications as graphs of operators that, step by step, transform data into the desired results. As operators can be deployed and executed independently, the DataFlow model supports parallelism and distribution, thus making streaming applications scalable. Today, we witness an abundance of SPEs, each with its set of operators. In this context, understanding how operators' semantics overlap within and across SPEs, and thus which SPEs can support a given application, is not trivial. We tackle this problem by formally showing that common operators of SPEs can be expressed as compositions of a single, minimalistic Aggregate operator, thus showing any framework able to run compositions of such an operator can run applications defined for state-of-the-art SPEs. The Aggregate operator only relies on core concepts of the DataFlow model such as data partitioning by key and time-based windows, and can only output up to one value for each window it analyzes. Together with our formal argumentation, we empirically assess how an SPE that only relies on such an operator compares with an SPE offering operator-specific implementations, as well as study the performance impact of a more expressive Aggregate operator by relaxing the constraint of outputting up to one value per window. The existence of such a common denominator not only implies the portability of operators within and across SPEs but also defines a concise set of requirements for other data processing frameworks to support streaming applications.

==> sections/checklist.tex <==
\section{CHECKLIST BEFORE SUBMISSION}

\begin{itemize}
    \item Do not differentiate between native and user-defined operators in terms of the latter allowing to define the semantics, because the former allow that too. Also, if eventually we show an Aggregate can really do a lot, is it fair to say it is less ``semantically powerful" than something else? OK
    % \item Do we actually use $\valuesof{t}$?
    \item Check that we use $A$ for Aggregate and $a$ for attribute OK
    \item the official format for stateful operators is $S_O = O(\WA,\WS,\keybysingle{},f_1,f_2)$ OK
    %% Following version had WO
    % \item the official format for stateful operators is $S_O = O(\WO,\WA,\WS,\keybysingle{},f_1,f_2)$
    \item The subsubindexes are like $S_{I_1}$ not $S_{I1}$ OK
    \item use macros in the entire paper, no handwritten symbols OK
    \item do we want to discuss space/time complexities for our solutions OK
    \item since our graphs can be cyclic, use the term query, not the term DAG in the paper OK
    \item Sometimes we use the notation $1, 2, \ldots$ sometimes $1, \ldots, n$, be uniform. OK
    \item use $=$ for checking equality and $\xleftarrow{}$ for assignment. OK
    \item output or emit OK
    \item do not user mathbin OK
    \item Do not use negative indexes for $t$ (if any) OK
    \item Do not use $i:$ notation OK
    \item This notation has been removed because it was never used $\langle \zeta,l,k \rangle$, and $k$ has also been removed since it was not used. Double-check OK
    \item WO has been removed because we were only using it for more complex operators, right? OK
    \item doublecheck for overloaded notation. We can assume $X$ and X are not overloaded? OK
    \begin{itemize}
        \item $A$ for aggregate and A for assumption, overloaded? OK
        \item $L$ for Allowed Lateness and L for code line, overloaded? OK
    \end{itemize}
    \item make sure spaces before/after symbols in math mode (e.g., colons) are consistent OK
    \item Make sure we use ingresses/egresses all over, not sources/sinks (or use the others, but be consistent) OK
    \item The following sentence is no longer needed in principle, but double-check: \textit{We say a window instance is \textit{expired} if its right boundary falls before the operator instance's watermark. We say a tuple is expired if it only contributes to expired window instances.} OK
    \item Notice that all code/discussion for now is for parallelism 1, what really happens if you increase parallelism remains to be checked OK
    \item eventually check all assumptions are used in the text (maybe not needed for SPE related assumptions?) OK
    \item First time you introduce Flink say Apache Flink + citation and then say simply Flink. Applies to other tools too. OK
    \item possible extension: Maybe also for different tuple sizes in the evaluation? OK
    \item possible extension: whole query in the evaluation? OK
    \item operators names with capital letter OK
    \item removed this because I think it is not needed ``, while $t[i:j]$ denotes the list of attributes from $i$ to $j$ (inclusive)." from the preliminaries OK
    \item removed ``If $\WA>\WS$, $\Window$ is called \textit{jumping} and each tuple falls in zero or one window instances." from prels, we do not use it OK
    \item type not schema!!!! OK
\end{itemize}
